$\text{Di}^2\text{Pose}$: Discrete Diffusion Model for Occluded 3D Human Pose Estimation

Continuous diffusion models have demonstrated their effectiveness in addressing the inherent uncertainty and indeterminacy in monocular 3D human pose estimation (HPE). Despite their strengths, the need for large search spaces and the corresponding demand for substantial training data make these models prone to generating biomechanically unrealistic poses. This challenge is particularly noticeable in occlusion scenarios, where the complexity of inferring 3D structures from 2D images intensifies. In response to these limitations, we introduce the Discrete Diffusion Pose ($\text{Di}^2\text{Pose}$), a novel framework designed for occluded 3D HPE that capitalizes on the benefits of a discrete diffusion model. Specifically, $\text{Di}^2\text{Pose}$ employs a two-stage process: it first converts 3D poses into a discrete representation through a \emph{pose quantization step}, which is subsequently modeled in latent space through a \emph{discrete diffusion process}. This methodological innovation restrictively confines the search space towards physically viable configurations and enhances the model's capability to comprehend how occlusions affect human pose within the latent space. Extensive evaluations conducted on various benchmarks (e.g., Human3.6M, 3DPW, and 3DPW-Occ) have demonstrated its effectiveness.

==> algorithm/alg1.tex <==
\begin{algorithm}[t]
\caption{Training of the $\text{Di}^2\text{Pose}$ model.}
\label{alg:PA1}
\begin{algorithmic}[1]
\REQUIRE ~~\\
    A transition matrix $\mathbf{M}_s$, the number of timesteps $S$, network parameters $\theta$, training epoch $M$, pose dataset $\boldsymbol{D}$ (including 2D image $I$ and 3D human pose $\mathbf{P}$), and the well-learned pose encoder $f_{PE}$.
    \FOR{$i=1$ to $M$}
    \FOR{$(I,\mathbf{P})$ in $ \boldsymbol{D}$}
    % \STATE $\boldsymbol{s} = \mbox{pose\_encoder(3D pose)}$;
    \STATE $\mathbf{k}_0 = f_{PE}$($\mathbf{P}$), $\boldsymbol{y}=$ImageEncoder($\mbox{I}$);
    \STATE sample $s$ from Uniform($1, 2, 3, ..., S$);
    \STATE sample $\mathbf{k}_s$ from $q(\mathbf{k}_s|\mathbf{k}_0)$ based on formula (\ref{formula:quick cal uniform and mask matrix});
    \STATE estimate $f_{\theta}(\mathbf{k}_{s-1}|\mathbf{k}_s,\boldsymbol{y})$;
    \STATE calculate loss according to formula (\ref{vlb loss}-\ref{diffu final loss});
    \STATE update network $\theta$;
    \ENDFOR
    \ENDFOR
\RETURN network $\theta$.
\end{algorithmic}
\end{algorithm}


==> algorithm/alg2.tex <==
\begin{algorithm}[t]
\caption{Inference of the $\text{Di}^2\text{Pose}$ model.}
\label{alg:PA2}
\begin{algorithmic}[1]
\REQUIRE ~~\\
    Time stride $\Delta_s$, the number of timesteps $S$, input text, the pose decoder $f_{PD}$, network $\theta$, stationary distribution $p(\mathbf{k}_S)$;
    \STATE $s=S$, $\boldsymbol{y}=$ImageEncoder(2D image);
    \STATE sample $\mathbf{k}_s$ from $p(\mathbf{k}_S)$;
    \WHILE{$s \textgreater 0$}
    \STATE $\mathbf{k}_s \leftarrow $ sample from $p_{\theta}(\mathbf{k}_{s-\Delta_s}|\mathbf{k}_s,\boldsymbol{y})$
    \STATE $s \leftarrow (s-\Delta_s)$
    \ENDWHILE
\RETURN  $f_{PD}(\mathbf{k}_s)$.
\end{algorithmic}
\end{algorithm}

